Truthful Mechanisms with Implicit Payment Computation

It is widely believed that computing payments needed to induce truthful bidding is somehow harder than simply computing the allocation. We show that the opposite is true: creating a randomized truthful mechanism is essentially as easy as a single call to a monotone allocation rule. Our main result is a general procedure to take a monotone allocation rule for a single-parameter domain and transform it (via a black-box reduction) into a randomized mechanism that is truthful in expectation and individually rational for every realization. The mechanism implements the same outcome as the original allocation rule with probability arbitrarily close to 1, and requires evaluating that allocation rule only once. We also provide an extension of this result to multi-parameter domains and cycle-monotone allocation rules, under mild star-convexity and non-negativity hypotheses on the type space and allocation rule, respectively. Because our reduction is simple, versatile, and general, it has many applications to mechanism design problems in which re-evaluating the allocation rule is either burdensome or informationally impossible. Applying our result to the multi-armed bandit problem, we obtain truthful randomized mechanisms whose regret matches the information-theoretic lower bound up to logarithmic factors, even though prior work showed this is impossible for truthful deterministic mechanisms. We also present applications to offline mechanism design, showing that randomization can circumvent a communication complexity lower bound for deterministic payments computation, and that it can also be used to create truthful shortest path auctions that approximate the welfare of the VCG allocation arbitrarily well, while having the same running time complexity as Dijkstra's algorithm.

==> app-prelims-old.tex <==
\section{Preliminaries}
\label{sec:prelims}

\xhdr{Single Parameter Domains.}
We present the single parameter model for which we apply our procedure. The model is very similar to the model of Archer and Tardos~\cite{ArcherTardos}, yet it is slightly more general. We state the model is terms of values and not costs and allow the values to be both positive and negative. We also allow randomization by nature. All these changes are minor and do not change the fundamental characterization, yet are helpful to later derive our results.


Let $n$ be the number of agents and let $N=[n]$ be the set of agents.
Each agent $i\in N$ has some private {\em type}
consisting of a single parameter $t_i\in T_i$ that describes
the agent, and is known only to $i$, everything else is public knowledge.
We assume that the domain $T_i$ is an open subset of $\Re$ which is an interval with positive length (possibly starting from $-\infty$ or going up to $\infty$).
Let $T=T_1\times T_2\times ... \times T_n$ denote the domain of types and let $t\in T$ denote the vector of true types.

There is some set of {\em outcomes} $O$.
For single-parameter domains, agents evaluate outcomes in a particular way that we describe next.
For each agent $i\in N$ there is a function $a_i:O\rightarrow \Re_{+}$ specifying the {\em allocation to agent $i$}.
The {\em value} of an outcome $o\in O$ for an agent $i\in N$ with type $t_i$ is $t_i\cdot a_i(o)$.
The {\em utility} that agent $i\in N$ derives from outcome $o\in O$ when he is charged $p_i$ is quasi-linear:
$u_i = t_i\cdot a_i(o) - p_i$.
%(In Economics literature, this is called ``quasi-linear utility".)

For instance, consider the allocation of $k$ identical units of good to agents with additive valuations:
agent $i$ has a value of $t_i$ {\em per unit}. An outcome $o$ specifies how many items each agent receives: $a_i(o)$ is the number of items $i$ receives. His valuation for that outcome is his value per-unit times the number of units he receives.

A (direct revelation) deterministic {\em mechanism} $\mathcal{M}$ consists of the pair $(\mA, \mP)$,
where $\mA:T\rightarrow O$ is the {\em allocation rule} and $\mP:T\rightarrow \Re^n$ is the {\em payment rule}, i.e. the vector of payment functions $\mP_i:T\rightarrow \Re$ for each agent $i$.
Each agent is required to report a type $b_i\in T_i$ to the mechanism, and $b_i$ is called the {\em bid} of agent $i$.
We denote the vector of bids by $b\in T$.
The mechanism picks an outcome $\mA(b)$ and charges agent $i$ payment of $\mP_i(b)$.
The allocation for agent $i$ when the bids are $b$ is $\mA_i(b)= a_i(\mA(b))$ and he is charged $\mP_i(b)$.
Agent $i$'s utility when the agents bid $b\in T$ and his type is $t_i\in T_i$ is
\begin{equation}\label{eq:util-det}
u_i(t_i,b) =  t_i\cdot \mA_i(b) - \mP_i(b)
\end{equation}

% To simplify notation, when the allocation rule is clear from the context, we will use $a_i(b)$ to denote $a_i(A(b))$, the allocation to $i$.

 We also consider randomized mechanisms, which are distribution over deterministic mechanisms. For a randomized allocation rule $\mA_i(b)$ and $\mP_i(b)$ will denote the {\em expected} allocation and payment charged from agent $i$, when the bids are $b$. The expectation is taken over the randomness of the mechanism. Sometimes it will be helpful to explicitly consider the deterministic allocation and payment that is generated for specific random seed. in this case we use $\rM$ to denote the random seed and use $\mA_i(b;\rM)$ and $\mP_i(b;\rM)$ to denote allocation and payment when the seed is $\rM$.

There may be some outside randomization that influences the outcome and is not controlled by the mechanism, e.g. randomness in the realization of clicks in sponsored search auction. We call this randomization by {\em nature}.  With such randomization  $\mA_i(b)$ and $\mP_i(b)$ also encapsulate expectations over nature's randomization. Finally, we use the notation $\eAAi{b}$ and $\ePPi{b}$ to denote the allocation and payment charged from agent $i$, when the bids are $b$, the mechanism random seed is $\rM$ and nature's random seed is $\rN$.
\cout{
We allow the allocation and payment rules to be randomized and also allow nature to randomize (meaning that the outcome might depend on nature randomization) and assume that agent are risk neutral, each aims to
maximize his expected utility.
Formally, an allocation rule $A$ is a function that takes bids $b$ and a random seed $\rA$ and outputs a distribution over outcomes (with randomness coming from nature), $A(b;\rA)\in \Delta(O)$, where $\Delta(O)$ is the space of probability distributions over outcomes $O$. Alternatively, fixing $b$ and $\rA$ we can also think of the allocation as a deterministic function of nature randomness $\rN$.
We denote that allocation with bids $b$, allocation random seed $\rA$ and nature random seed $\rN$ as $\A{b}\in O$.
Now $\Aii{b}$ denotes the allocation to agent $i$, that is  $\Aii{b} = a_i(\A{b})$.
Similarly, the payment rule might be randomized with random seed $\rP$, and we can denote
the deterministic payment of agent $i$ when the bids are $b$, its random seed is $\rP$ and nature random seed is $\rN$ by $\Pii{b}\in \Re$. % \mbcomment{Is this the formulation we want ?}
Agent $i$'s utility when the agents bid $b$ and his type is $t_i$ is

\begin{equation}\label{eq:util}
u_i(t_i,b) =  \E_{\rA,\rP,\rN}\left[ t_i\cdot \Aii{b} - \Pii{b} \right]
\end{equation}

Note that the expectation is over all randomness (nature and rules).\footnote{One can also consider Bayesian settings in which agents have a prior over the types of others and try to maximize the expected utility, where expectation is taken also over the randomization generating the types of the others (rather than for a fixed $b_{-i}$). Our framework and results can be easily extended to this case, by capturing any such randomness similarly to the way we capture other randomness by nature and taking expectation of this randomness as well.}
} % cout

\xhdr{Allocation and Mechanism Properties.}
Let $b_{-i}$ denote the vector of bids of all agents but agent $i$. We can now write the vector of bids as $b=(b_{-i}, b_i)$. Similar notation will be used for other vectors.

We next list two central properties, truthfulness and individual rationality.
\begin{itemize}
\item
Mechanism $\mathcal{M}$ is {\em truthful} if for every agent $i$ truthful bidding is a {\em dominant strategy}: for every agent $i$, bidding $t_i$ always maximizes her utility,
regardless of what the other agents bid.
Formally,
\begin{equation}\label{eq:truthful}
%u_i(t_i,(b_{-i}, t_i)) =
t_i\cdot \AAi{b_{-i}, t_i} - \PPi{b_{-i}, t_i} \ge t_i\cdot \AAi{b} - \PPi{b}
% u_i(t_i, (b_{-i}, t_i)) \ge u_i(t_i, (b_{-i}, b_i))
\end{equation}
holds % , in expectation over $\rA,\rP$ and $\rN$,
for every agent $i\in N$, type $t_i\in T_i$, bids of others $b_{-i}\in T_{-i}$ and bid $b_i\in T_i$ of agent $i$.
\item Mechanism $\mathcal{M}$ is {\em individually rational (IR)} if an agent never receives negative utility by participating in the mechanism and bidding truthfully. Formally,
    % for every agent $i$, type $t_i$ and every bids $b_{-i}$, an agent who bid truthfully never incurs a net loss, i.e.
    \begin{equation}\label{eq:ir}
    t_i\cdot \AAi{b_{-i}, t_i} - \PPi{b_{-i}, t_i} \ge 0
    % u_i(t_i, (b_{-i}, t_i)) \ge 0
    \end{equation}
    holds %, in expectation over $\rA,\rP$ and $\rN$,
    for every agent $i\in N$, type $t_i\in T_i$ and bids of others $b_{-i}\in T_{-i}$.
\end{itemize}

It will be helpful to establish terminology for the case that the above hold not only in expectation but also for specific realizations. For example, we will say that a mechanism is {\em universally truthful} if \refeq{eq:truthful} holds not only in expectation over the mechanism's randomness, but rather for every realization of that randomness. In general, every property that we define is defined by some inequality, and if the inequality holds for every realization of the mechanism randomness we say that it holds {\em universally}, and if it holds for every realization of nature randomness we say that it holds {\em ex-post}. When we want to emphasize that the property holds only in expectation over the nature's randomness we say that it holds {\em stochastically}.

\cout{
As we have multiple sources of randomness it will be helpful to establish some terminology for quantifiers over the different randomness sources. A given property $p$ will be defined by some inequality.
For a given property $p$, we say that $p$ {\em holds} if the inequality holds in expectation over all sources of randomness.
The property holds {\em ex-post} if the inequality holds for every realization of nature randomness.
The property holds {\em universally} if the inequality holds for every realization of the mechanism randomness.
Thus, $p$ holds universally and ex-post if the inequality holds for every realization of both nature and the mechanism randomness.

Note that if nature does not randomize and the mechanism is deterministic the above properties hold both universally and ex-post.
}

% If truthful bidding is a dominant strategy for all agents we say that the mechanism is {\em truthful}.

% Mechanism $M$ is {\em individually rational (IR)} if for every agent $i$ with any type $t_i$ and for every bids $b_{-i}$, an agent who bid truthfully never incurs a net loss, i.e. $u_i(t_i, (b_{-i}, t_i)) \ge 0$.
Note that in an individually rational mechanism an agent is ensured not to incur any loss {\em in expectation}.
That is rather unsatisfying as for some realizations the agent might suffer a huge loss.
It is more desirable to design mechanisms that are {\em universally ex-post individually rational}, that is
% Thus we consider a refined condition. When the utility of an agent is a random variable (due to nature's randomness or the mechanism's randomness) the mechanism is {\em ex-post individually rational} if for every $i, t_i, b_{-i}, \rA, \rP$ and $\rN$,
% it holds that $$t_i\cdot A_i((b_{-i}, t_i), \rA, \rN) - P_i((b_{-i}, t_i), \rP,\rN)\ge 0$$ That is,
a truthful agent should incur no loss for every bids of the others and {\em every realization} of the random events (not only in expectation).

% An allocation rule $\mA$ {\em admits a truthful payment rule} if there exists a payment rule $\mP$ such that the mechanism $M = (\mA, \mP)$ is truthful.

If all types are positive, then in addition to individual rationality it is desirable that all agents are charged a non-negative amount; this is known as the \emph{\noPositiveTransfers} property.
\OMIT{ %%%%%%%%%%%%%
If all types are positive, a stronger property is desirable (and satisfied by~\refeq{eq:myerson}): a mechanism is called \emph{normalized} if it is individually rational and moreover all agents are charged a non-negative amount.
} %%%%%%%%%%
Finally, the \emph{welfare} of a truthful mechanism is defined to be the total utility
	$\sum_i t_i \cdot \mA_i(t)$.


\xhdr{Characterization.}
The following characterization of truthful mechanisms, due to Archer and Tardos~\cite{ArcherTardos}, is almost identical to the characterization presented by Myerson~\cite{Myerson} for truthful mechanisms in the special case of single item auctions. The crucial property of an allocation that yields truthfulness is \emph{monotonicity}, defined as follows:

\begin{definition}\label{def:mon}
Allocation rule $\mA$ is {\em monotone} if for every agent $i\in N$, bids $b_{-i}\in T_{-i}$ and two possible bids of $i$, $b_i\ge b^{-}_i$, we have
$\AAi{b_{-i}, b_i}\ge  \AAi{b_{-i}, b^{-}_i}$.
\end{definition}
Recall that monotonicity of an allocation rule is also defined universally and/or ex-post.

We next present the characterization of truthful mechanisms.  In the theorem statement, the
expression $\AAi{b_{-i},u}$ is interpreted to equal zero when $u \not\in T_i.$

\begin{theorem}\label{thm:myerson}~\cite{Myerson,ArcherTardos}
Consider a single-parameter domain. An allocation rule $\mA$ admits a payment rule $\mP$ such that the mechanism $(\mA,\mP)$ is truthful if and only if $\mA$ is monotone and moreover for each agent $i$ and bid vector $b$
it holds that
 $ \int_{-\infty}^{b_i} \AAi{b_{-i}, u} \,du < \infty$.
In this case the payment for each agent $i$ must satisfy
\begin{align}\label{eq:myerson}
\PPi{b}  =
 \mP_i^0(b_{-i}) +
 b_i\, \AAi{b_{-i}, b_i} -
 \textstyle{\int^{b_i}_{-\infty}}\,  \AAi{b_{-i}, u} \,du,
\end{align}
where $\mP_i^0(b_{-i})$ does not depend on $b_i$.
\end{theorem}

<<<<<<< app-prelims.tex
A mechanism is called \emph{normalized} if zero allocation implies a zero payment.
=======
A mechanism is called \emph{normalized} if for each agent $i$ and every bid vector $b$, zero allocation implies a zero payment:
	$\AAi{b}=0 \Rightarrow \PPi{b}=0$.
>>>>>>> 1.11

\begin{corollary}\label{cor:myerson}
The truthful mechanism in Theorem~\ref{thm:myerson} is normalized if and only if $\mP_i^0(b_{-i}) \equiv 0$, in which case the mechanism is also individually rational and (for positive-only types) satisfies the no-positive-transfers property.
\end{corollary}

\OMIT{
\begin{theorem}\label{thm:myerson}~\cite{Myerson,ArcherTardos}
A monotone allocation rule $\mA$ admits a payment rule $\mP$ such that the mechanism $(\mA,\mP)$ is truthful and individually rational if and only if
% $ \int_{-\infty}^{\infty} \E_{\rA,\rN}\left[ \Aii{(b_{-i}, u)}\right] du < \infty$
for each agent $i$ and bid vector $b$
	$ \int_{-\infty}^{b_i} \AAi{b_{-i}, u} \,du < \infty$
In this case
\begin{align}\label{eq:myerson}
\PPi{b}  = b_i \AAi{b_{-i}, b_i} - \textstyle{\int^{b_i}_{-\infty}}\,  \AAi{b_{-i}, u} \,du.
\end{align}
\end{theorem}
<<<<<<< app-prelims.tex
Note that if $\mA$ is ex-post monotone then the mechanism is ex-post truthful and ex-post individually rational.
=======
}

<<<<<<< app-prelims.tex
\begin{remark}
Both Theorem~\ref{thm:myerson} and Corollary~\ref{cor:myerson} hold in the ``ex-post" sense (resp., ``universal" sense), if  $\mA_i$, $\mP_i$ and $\mP^0_i(b_{-i})$ are interpreted to mean the respective values for a specific random seed of nature (resp., mechanism).
\end{remark}
>>>>>>> 1.7
% Moreover, if all types are positive then the mechanism is normalized.
<<<<<<< app-prelims.tex
=======
>>>>>>> 1.11

<<<<<<< app-prelims.tex
New 11111111111111:
\begin{theorem}\label{thm:myerson}~\cite{Myerson,AT01}
An allocation rule $\mA$ admits a payment rule $\mP$ such that the mechanism $(\mA,\mP)$ is truthful if and only if $\mA$ is monotone and moreover for each agent $i$ and bid vector $b$
	$ \int_{-\infty}^{b_i} \AAi{b_{-i}, u} \,du < \infty$.
In this case the payment must be
\begin{align}\label{eq:myerson}
\PPi{b}  =
	\mP_i^0(b_{-i}) +
	b_i \AAi{b_{-i}, b_i} -
	\textstyle{\int^{b_i}_{-\infty}}\,  \AAi{b_{-i}, u} \,du, 
\end{align} 
where the term $\mP_i^0(b_{-i})$ depends only on $b_{-i}$, but not on $b_i$. The mechanism is $0$-normalized if and only if this term is $0$, in which case it is also individually rational.
\end{theorem}=======

Note that for Corollary~\ref{cor:myerson} to apply, truthfulness and normalization must hold in the same ``sense", e.g. both ex-post.  >>>>>>> 1.7
=======
Both Theorem~\ref{thm:myerson} and Corollary~\ref{cor:myerson} hold in the ``ex-post" sense (resp., ``universal" sense), if  $\mA_i$, $\mP_i$ and $\mP^0_i(b_{-i})$ are interpreted to mean their respective values for a specific random seed of nature (resp., mechanism). In Corollary~\ref{cor:myerson}, the mechanism is normalized in the same sense as it is truthful.>>>>>>> 1.11

